OpenM3D: Open Vocabulary Multi-view Indoor 3D Object Detection without Human Annotations

Open-vocabulary (OV) 3D object detection is an emerging field, yet its exploration through image-based methods remains limited compared to 3D point cloud-based methods. We introduce OpenM3D, a novel open-vocabulary multi-view indoor 3D object detector trained without human annotations. In particular, OpenM3D is a single-stage detector adapting the 2D-induced voxel features from the ImGeoNet model. To support OV, it is jointly trained with a class-agnostic 3D localization loss requiring high-quality 3D pseudo boxes and a voxel-semantic alignment loss requiring diverse pre-trained CLIP features. We follow the training setting of OV-3DET where posed RGB-D images are given but no human annotations of 3D boxes or classes are available. We propose a 3D Pseudo Box Generation method using a graph embedding technique that combines 2D segments into coherent 3D structures. Our pseudo-boxes achieve higher precision and recall than other methods, including the method proposed in OV-3DET. We further sample diverse CLIP features from 2D segments associated with each coherent 3D structure to align with the corresponding voxel feature. The key to training a highly accurate single-stage detector requires both losses to be learned toward high-quality targets. At inference, OpenM3D, a highly efficient detector, requires only multi-view images for input and demonstrates superior accuracy and speed (0.3 sec. per scene) on ScanNet200 and ARKitScenes indoor benchmarks compared to existing methods. We outperform a strong two-stage method that leverages our class-agnostic detector with a ViT CLIP-based OV classifier and a baseline incorporating multi-view depth estimator on both accuracy and speed.

==> sections/method/01_pseudo_3D_box.tex <==
\subsection{3D Pseudo Box Generation}\label{sec.m-3dbox}
% [overview of generating pseudo boxes]
%Precise object localization is fundamental for object detection.
%
% \tao{To produce class-agnostic bounding boxes for OV-ImGeoNet's training, we propose to (1) lift class-agnostic 2D image segmentation from SAM~\cite{SAM} into 3D and (2) merge various viewpoints through a graph embedding-based method that considers view consistency.}
\input{figures/gen_pseudo_box}
To train the class-agnostic 3D object detector of {\ourmethod}, we generate generic 3D pseudo boxes.
% To train {\ourmethod}'s class-agnostic detector, we apply 3D pseudo-box generation to unlabeled training data to ensure high precision and recall for all objects.
%

Our approach consists of (1) utilizing a class-agnostic 2D segmenter to generate partial 3D segments by lifting the 2D segment results into 3D, and (2) completing the 3D segments by merging these partial 3D segments from various viewpoints through a graph embedding-based method. Fig.~\ref{fig:gen_pseudo_box} shows the proposed 3D pseudo box generation overview.
%
% [How to get segments from SAM and the 3D projection]

\noindent\textbf{Partial 3D Segments (Fig.~\ref{fig:gen_pseudo_box}~(a,b)).}
%%
% \tao{multi-view $\rightarrow$ 2D RGB images of various viewpoints.}
Given an RGB image $I$, we extract the 2D segments $n_{j}^{\text{2D}}$ of the whole scene $S^{\text{2D}}=\{n_{j}^{\text{2D}}\}$ using an off-the-shelf class-agnostic 2D instance segmentation approach, where each 2D segment contains a set of pixel positions $\{(u, v)_q\}$. 
% $S^{\text{2D}} = \{ n^{\text{2D}}_j\}$ consists of many segments indexed by $j$ and each segment $n^{\text{2D}}_j = \{(u, v)_q\}$ consists of many pixel positions $(u,v)$ indexed by $q$. 
% For each 2D segment $n^{\text{2D}}_j$, we use the corresponding depth map $D$ and camera pose to lift it to a partial 3D segment $n^{\text{3D}}_j = \{(x, y, z)_q\}$ consists of many 3D points $(x,y,z)$ as follows,
Subsequently, we lift each 2D segment into 3D based on the provided camera pose $(\mdmat{R}, \mdmat{t})$, intrinsic $\mdmat{K}$, and depth map $\mdmat{D}$ by
\begin{equation} \label{eq:projection}
    \begin{bmatrix}
        x \\
        y \\
        z 
    \end{bmatrix}
    =\mdmat{R}^T \mdmat{K}^{-1} \mdmat{D}(u,v)
    \begin{bmatrix}
        u \\
        v \\
        1 
    \end{bmatrix}
    -
    \mdmat{R}^T \mdmat{t}~.
\end{equation}
We denote the result of \mdeq{\ref{eq:projection}} as a partial 3D segment $n^{\text{3D}}_j = \{(x, y, z)_q\}$, comprising numerous 3D points $(x, y, z)$, as it only includes partial observation from a single view. 
% Note that a partial 3D segment corresponds to the visible surface of a 3D object from the RGB image.
% To utilize information from various viewpoints, we explore methods for aggregating 3D partial segments. However, aggregating these segments is challenging due to inherent noise from imperfect 2D segments. The goal is to merge these noisy partial 3D segments from different views into a more robust and complete 3D representation.
% While aggregating partial 3D segments across multiple views is the most intuitive way to complete the surface of a 3D object, achieving robust aggregation without amplifying noise and bias is non-trivial.
To incorporate information from multiple viewpoints, we explore methods for aggregating 3D partial segments, 
though this process is complicated by noise from imperfect 2D segments. 
The goal is to merge these noisy partial segments into a more robust 3D representation. 
While aggregating partial segments across views is intuitive for completing a 3D object's surface, 
achieving this without amplifying noise and bias remains challenging.
%Given $N$ RGB images, $\mathbb{I}=\{I_t\}_{t=1}^N \subseteq {\mathbb{R}}^{H \times W \times 3}$, along with extrinsics, $\mathbb{P}=\{P_t\}_{t=1}^N$, in a scene, we firstly extract the corresponding segmentation maps $\mathbb{S}^{2D}=\{S^{2D}_t\}_{t=1}^N$ with an off-the-shelf class-agnostic 2D instance segmentation approach \fuen{cite or just use the name}. Within each segmentation map $S^{2D}_t \subseteq {\mathbb{Z}}^{H \times W}$, every integer corresponds to a distinct segment.Then, we leverage their depth maps $\mathbb{D}=\{D_t\}_{t=1}^N$ and lift these 2D segmentation maps to 3D partial segments $\mathbb{\hat{S}}^{3D}=\{\hat{S}^{3D}_t\}_{t=1}^N$, ${\hat{S}^{3D}_{t}} = \{n_{i}^{t}\}_{i=0}^M$:

% where n_i^{t}$ includes the point set along with segment index $i$,  

%
% \tao{why mention NODE here? It should be in next apart?.}
% Each segment corresponds to an instance, which represents a node in the following graph embedding-based method. 
% %
% \tao{The filtering mechanism can be moved to implementation details.}
% Besides, to mitigate the impact of background elements such as the floor, walls, and ceiling, which can potentially introduce errors in graph embedding due to their substantial spatial presence, we harness MaskDINO~\cite{li2022mask} to filter out the background effectively.
%
% \tao{project $\rightarrow$ back-project}
%Within every 2D mask \mdineq{\mdmat{M}_{\text{2D}} \subseteq {\mathbb{Z}}^{H \times W}}, each pixel $(u, v)$ is back-projected into 3D space as follows:
% \tao{Use one SE(3) matrix to represent rotation and translation, please refer to Imgeonet's eq 3}
%
% \Pi change
%where \mdineq{(x, y, z)} represents the back-projected 3D coordinate, \mdineq{\mdmat{d}} represents the per-pixel depth, \mdineq{\mdmat{K} \subseteq {\mathbb{R}}^{3 \times 3}} stands for the camera intrinsic matrix, and \mdineq{\mdmat{R}} and \mdineq{\mdmat{t}} denote rotation matrix and translation vector, respectively, of the camera pose.
%
%For each 3D point set back-projected from the 2D mask, we denote it as a 3D partial mask \mdineq{\mdmat{M_{\text{3D}}}}, representing 2D class-agnostic segment results in 3D.

%Since minor variations of 3D point coordinates may arise due to noises in depth maps, we standardize the coordinates across all 3D partial segments by utilizing voxelization followed by K-nearest neighbors (KNN) to fuse 3D points to the vertices extracted from the ground truth mesh.

%When representing an instance using 3D partial masks from various viewpoints, minor variations in point coordinates may arise. 
%
%To standardize the coordinates in each 3D partial mask, we utilize voxelization followed by K-nearest neighbors (KNN) to fuse 3D points to the vertices extracted from the ground truth mesh.
%
%Specifically, we fuse the point set within each voxel grid to the nearest extracted vertex determined by KNN.
%
%This process unifies the coordinates in 3D partial masks from various viewpoints. 
%However, since the 2D instance segmenter produces inconsistent results across different viewpoints, we introduce ``View Consistent 3D Segments'' through a graph embedding-based clustering technique to integrate segments from different views.
%\fuen{To PH: why graph embedding can solve this, plz add description. The connection of graph embedding and following parts are not clear.}
% \tao{(1) KNN and voxelization should be 2 different things, please explain separately. Make sure we clarify our motivation to use them. (2) This sentence is not pellucid enough: "thereby representing an entire scene from a single frame." (3) what is the scene mesh?}
% \peng{Subsequently, we employ the K-nearest neighbors (KNN) to combine each projected 3D point with the nearest vertex extracted from the scene mesh, thereby representing an entire scene from a single frame. 
% %
% \peng{predefine grid --> KNN by this predefined grid}
% After back-projection, a grid pooling method [xxx] is applied to downsample 3D points.
%
% By inheriting per-pixel 2D masks from SAM, we can obtain per-point 3D masks \mdineq{M^{i}_{3D}}
% \peng{2D masks --> point-set --> we denote it as 3D mask}

%
% \tao{this part is a little confusing. what is a 3D mask?}
% For frame \(i\), the entire 3D mask can be expressed as \(M^{i}_{3D} = \left\{ m_{1}^{i}, m_{2}^{i}, ..., m_{n}^{i} \right\}\), where \(m\) stands for segment ids, and \(n\) is the number of points in the scene.}

%
% \tao{Make it concise: However, since SAM produces inconsistent results across adjacent views, we introduce \emph{Graph Embedding-Based Clustering} ...}
% \peng{However, aggregating multi-view results becomes challenging due to inconsistent SAM results across adjacent views. Therefore, to properly integrate segments from each frame, we introduce \emph{Graph Ebedding-Based Clustering}.}
%
%However, since the 2D instance segmenter produces inconsistent results across adjacent views, we introduce \emph{Graph Embedding-Based Clustering} to integrate segments from different views.
%%

\noindent\textbf{Complete 3D Segments (Fig.~\ref{fig:gen_pseudo_box}~(c,d,e)).}
%Graph-Based Clustering for
% Sequentially aggregating the partial segments is likely to accumulate errors since segments from multiple views are not considered simultaneously.
% A straightforward sequential aggregation of partial segments tends to accumulate errors.
% %
% This occurs because the aggregation result, based on only a few consecutive frames from a previous time step, lacks complete object understanding, making it inherently noisy.
A simple sequential aggregation of partial segments accumulates errors due to incomplete object understanding. It relies on limited consecutive frames from a previous time step, resulting in inherent noise.
% Hence, we formulate the task as a graph embedding problem where each partial segment $n^{3D}_j$ is a node to enable simultaneous consideration of all views.
Hence, we propose a graph embedding-based method that considers all viewpoints simultaneously.
The scene is represented as a graph, with each node as a partial 3D segment $n^{3D}_j$, and edges indicating a high likelihood on nodes of the same object.
% Specifically, we represent a scene as a graph, where each node corresponds to a partial 3D segment $n^{3D}_j$.
% We aim to learn a representation for each node, expecting the edges to signify the similarity between nodes.
% , and edges between nodes indicate their spatial proximity.

%$n^{3D}_j$ and $n^{3D}_k$ are connected if their overlap ratio is high. Next, we use graph embedding-based clustering to group partial segments into a complete segment considering the part-wise connectivity of segments in the graph.
%aggregate segments from 3D across different viewpoints into individual instances. 
% 
%By leveraging the connectivity of the graph, we can link segments representing the same instance. This connectivity is then employed in graph embedding-based clustering to create a view-consistent 3D segment.
% \peng{why graph embedding? advantage?}
% This process involves (1)building a learning target (2) learning graph embedding, and (3) voting for final segmentation.
% To begin with, we employ an undirected graph structure to represent the connectivity among individual segments, where each partial 3D segment $n_{j}^{3D}$ is defined as a node.
% %
% We aim to create edges to link nodes belonging to the same instance.
%
%\tao{Simplify "Through voxelization ... determine the existence of edges"}
% To connect the nodes (i.e., segments) in the graph, 
To learn such graph representation, we apply an off-the-shelf graph embedding method on the graph data that considers the entire scene.
%
% The edge of this graph data is created if the overlap ratio between two nodes is high.
%
For a pair of nodes (\ie, partial segments) in this graph data, an edge is established when the overlapping ratio between two nodes exceeds a specific threshold \mdineq{\theta} as follows:
% To derive the graph for training, we need to determine the edges between nodes (i.e., segments).
% We apply voxelization for efficiency to pair nodes $(n^{\text{3D}}_{j}, n^{\text{3D}}_{k})$ within the same voxel grid and determine the existence of edge by
% Through voxelization, each voxel grid contains nodes with near spatial distance which tends to represent the same instance.
% %
% Within each voxel grid, nodes are paired with one another to determine the existence of edges.
%
% For node pair \mdineq{(X_{i}, X_{y})}, we calculate the edge by
\begin{align} \label{eq:bw_warp}
    &e_{jk} = \mathrm{edge}(n_{j}^{\text{3D}}, n_{k}^{\text{3D}}) = \begin{cases}
        1, & \text{if \mdineq{O(n_{j}^\text{3D}, n_{k}^\text{3D})}} > \theta,\\
        0, & \text{else}
    \end{cases} ~, \\
% \end{equation}
% \begin{equation} 
% \label{eq:overlap}
\label{eq:overlap}
&O(n_{j}^\text{3D}, n_{k}^\text{3D}) = \frac{|n_{j}^{\text{3D}}\bigcap n_{k}^{\text{3D}}|}{\text{min}(|n_{j}^{\text{3D}}|, |n_{k}^{\text{3D}}|)}
    % O = \frac{|n_{j}^{\text{3D}} \bigcap n_{k}^{\text{3D}}|}{\text{min}(|n_{j}^{\text{3D}}|, |n_{k}^{\text{3D}}|)}
\end{align}
% \begin{align}
% formula A \\
% formula B
% \end{align}
%
where $|\cdot|$ counts the number of points in a set, and $\bigcap$ denotes intersection of two sets.
We only consider the node pairs within the same voxel for efficiency.
%\tao{How to calculate \mdineq{\sigma_{\text{overlap}}}?}
%Additionally, \mdineq{\sigma_{\text{overlap}}} is the number of points overlapping in 3D coordinates between \mdineq{n_{j}^{3D}} and \mdineq{n_{k}^{3D}}.
% Through voxelization, all the edges can be computed efficiently. 
The final graph shows the interconnections between nodes (\ie, overlapping partial 3D segments) across the entire scene from multiple views.

%%
% \tao{What is the embedding here? I didn't see any previous parts for graph embedding...}
% \tao{Use concise statement.}
% Next, we want to learn a feature representation for each node (i.e., each partial 3D segment) such that tightly connected nodes share similar features.
%we acquire an embedding from the graph and employ clustering to group each node into specific instances.
%
% We apply an off-the-shelf graph embedding method 
% to extract our designed node feature.
%During the learning process, we can deduce the relationship between nodes: the more robust the connectivity, the shorter the embedding distance between a pair of nodes, signifying a higher likelihood that the pair of nodes belong to the same instance.
%\peng{TODO: connect to clustering}
%\peng{To leverage the information provided in the graph, we employ graph embedding further to quantify node similarity in the embedded vector space. 
%
%\tao{Use concise statement.}
% After obtaining node features from the off-the-shelf graph embedding method, complete 3D segments that account for partial object segments from all viewpoints can be generated by grouping similar nodes (\ie, partial segments) using K-Means.
\peng{After obtaining node features from the off-the-shelf graph embedding method, we generate complete 3D segments that account for partial object segments from all viewpoints by grouping similar nodes (\ie, partial segments) using K-Means.}
%
We then form a complete 3D segment by collecting all partial segments in the same cluster $q$ as follows $\hat{n}^{\text{3D}}_{q} = \{n^{\text{3D}}\in \mathcal{C}_{q}\},$
%\begin{equation} \label{eq:comseg}
%\hat{n}^{\text{3D}}_{q} = \{n^{\text{3D}}\in \mathcal{C}_{q}\},
%\end{equation}
where $\mathcal{C}$ is the set of partial 3D segments that share the same segment index of a clustered group $q$.

% 
%\tao{Clarify clustered result here. Use concise statement.}
%Each instance in the entire scene gets a unique segment ID from the clustered result.
%
%\tao{We update the segment ID w/ clustered results?}
%Then we map these new segment ID back to each frame.
%
%For frame $i$, the updated 3D mask is represented as \(\hat{M}^{i}_{3D} = \left\{ \hat{m}^{i}_{1}, \hat{m}^{i}_{2}, ..., \hat{m}^{i}_{n} \right\}\), where $\hat{m}$ denotes the clustered segment ID, and $n$ is the count of points in the scene.
%
%\tao{on voxelized space? clarify context here.}
%To account for 3D masks across all frames, we conduct per-point voting to determine the consolidated segment result of the entire scene.
%
%\tao{what is 3D segmentation result? what limitation? what is the idea of the connected-component algo? All too nebulous...}
%Due to the clustering method's limitations, we apply a connected-component algorithm to further refine the 3D segment result by separating far away points set among each segment ID.
%
%\tao{What is the result here? bbox? 3D semantic segmentation? what format?}
%Finally, we obtain the ultimate result in the graph embedding-based clustering method.
%
% \innersec{Ensemble with Over-segmentation.} % need to change
% \tao{Could we move this part to implementation details?}
% \tao{Why do we need to mention scannet here?}
% As mentioned in ScanNet~\cite{dai2017scannet}, there exists a normal-based graph cut method~\cite{felzenszwalb2004efficient} that takes mesh as the input to create conservative over-segmentation of the mesh. 
% %
% We aim to utilize this over-segmentation to further refine our graph embedding-based clustered result.
% % 
% \tao{Just say we use it and cite it, do NOT say similarly.}
% Similarly, we apply the conditional statement mentioned in \mdeq{\ref{eq:ovelapping}} to identify overlapping segments.
% %
% \tao{what statement?}
% When the statement holds, we use our segment results to replace the over-segmentation in the overlapping regions.
% %
% \tao{Delete this sentence.}
% By the refinement ensembled with over-segmentation, we can obtain a higher segmentation quality.
% %
% \tao{bound $\rightarrow$ generate or produce.}
% Next, we utilize this ensembled segmentation to bound pseudo 3D boxes.
% %
% %


\innersec{Mesh Segmentation Refinement.}
Besides our complete 3D segments derived from multi-view images, we can further consider the 3D segments $S^{\text{mesh}} = \{n^{\text{mesh}}_{j}\}$ that are generated by a mesh-based segmentation method.
% We can further incorporate our complete 3D segments derived from images with the 3D segments computed from ground truth meshes.
% Besides generating 3D segments from multi-view RGB images, we leverage ground truth meshes to refine the complete 3D segments.
%
Using ground truth mesh as input, we apply an off-the-shelf graph cut method~\cite{felzenszwalb2004efficient} to generate an additional set of 3D segments $S^{\text{mesh}}$.
%
To fuse these two kinds of 3D segments, that is $\{n^{\text{mesh}}_{j}\}$ and $\{\hat{n}^{\text{3D}}_{q}\}$, we apply \mdeq{\ref{eq:overlap}} to determine the overlapping ratio between any pairs of two segments from images and the mesh.
% Similarly, we view each segment $n^{\text{mesh}}_{j}$ as a node, and pair with each complete segment $\hat{n}^{\text{3D}}_{q}$ to compute edge by \mdeq{\ref{eq:bw_warp}}.
%
For each 3D segment $n^{\text{mesh}}_{j}$ from the mesh, we identify its overlapped 3D segment from our complete 3D segments $\hat{n}^{\text{3D}}_{h}$ with the highest overlapping ratio, and subsequently update the segment index in $n^{\text{mesh}}_{j}$ from $j$ to $h$.
%
By updating segment indices and combining 3D segments with the same segment index, we fuse the over-segmentation of the mesh to refine the original complete 3D segments back-projected from multi-view.% RGB images.

\innersec{3D Boxes from Complete 3D Segments.} 
To derive the axis-aligned 3D bounding box that encompasses each complete 3D segment $\hat{n}^{3D}_q$, 
we calculate the box center $(x,y,z)$ as the mean 3D position of the 3D segment in each axis direction, and the minimum and maximum coordinates in each direction to derive the width $w$, length $l$, and height $h$ of the 3D box.
%Given the ensembled 3D segmentation, we query points in each segment ID to bound axis-aligned boxes by the minimum and maximum value in each axis direction.
%
%\tao{Make it specific.}
Additionally, we apply thresholding on the volume of each 3D box and the number of points contained within each box to remove abnormally small or less visible boxes.

\input{figures/model}

==> tables/baseline_compare.tex <==
% \begin{table}[t]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Pipeline} & \textbf{Input Type} & \textbf{GPU Usage (GB)} & \textbf{Model Size} & \textbf{Inference Time (s)} \\
% \midrule
% VGGT + OVIR-3D & Recon + Posed RGB & 11.4 + 45.8 & $>$1.2B & $\sim$1.2 + $\sim$300 \\
% \textbf{OpenM3D (Ours)} & Posed RGB only & \textbf{12.5} & \textbf{159.4M} & \textbf{$\sim$0.3} \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:efficiency_comparison}
% \vspace{-15pt}
% \end{table}

\begin{table}[h]
\vspace{-6pt}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Pipeline} & \textbf{GPU Usage (GB)} & \textbf{Model Size} & \textbf{Inference Time (s)} \\
\midrule
VGGT + OVIR-3D & 11.4 + 45.8 & $>$1.2B & $\sim$1.2 + $\sim$300 \\
\textbf{OpenM3D (Ours)} & \textbf{12.5} & \textbf{159.4M} & \textbf{$\sim$0.3} \\
\bottomrule
\end{tabular}
}
\label{tab:efficiency_comparison}
\vspace{-6pt}
\end{table}

==> tables/pseudo_box_w_cropformer.tex <==
\begin{table}[t]
\small
\centering
  \caption{
  \textbf{3D Pseudo Box Evaluation with different 2D segmentation} on ScanNet200. 
While generating 3D pseudo boxes using different 2D segmentation sources in our method, we can obtain boxes with varying quality. For example, when CropFormer is applied, these boxes outperform all other methods in terms of precision and recall at IoU@0.25 and IoU@0.50.
}
\vspace{-0.5em}
    \begin{tabular}{@{}lccccc@{}}
    \toprule
    \multirowcell{2}[-0.6ex][l]{Method} &\multirowcell{2}[-0.6ex][c]{2DSeg} & \multicolumn{2}{c}{Precision (\%)} & \multicolumn{2}{c}{Recall (\%) } \\
    \cmidrule(l){3-4} \cmidrule(l){5-6}
    && \multicolumn{1}{c}{@0.25} & \multicolumn{1}{c}{@0.50} & \multicolumn{1}{c}{@0.25} & \multicolumn{1}{c}{@0.50}\\
    \midrule
    OV-3DET~\cite{lu2023openvocabulary} &Detic~\cite{Detic}& \multicolumn{1}{c}{11.62} & \multicolumn{1}{c}{4.40} & \multicolumn{1}{c}{21.13} & \multicolumn{1}{c}{7.99} \\
    SAM3D~\cite{yang2023sam3d} &SAM~\cite{SAM}& \multicolumn{1}{c}{14.48} & \multicolumn{1}{c}{9.05} & \multicolumn{1}{c}{57.7} & \multicolumn{1}{c}{36.07} \\
    \midrule
    \multirowcell{2}[-0.6ex][l]{Ours} &SAM~\cite{SAM}& \multicolumn{1}{c}{32.07} & \multicolumn{1}{c}{18.14} & \multicolumn{1}{c}{58.3} & \multicolumn{1}{c}{32.99} \\
     &CropFormer~\cite{qilu2023high}& \multicolumn{1}{c}{\textbf{35.58}} & \multicolumn{1}{c}{\textbf{22.72}} & \multicolumn{1}{c}{\textbf{62.60}} & \multicolumn{1}{c}{\textbf{39.97}} \\
    \bottomrule
    \end{tabular}
  \label{table:cropformer-scannet200-pseudo-box}%
\end{table}%
